DeepMask: an algorithm for cloud and cloud shadow detection in optical satellite remote sensing images using deep residual network

Detecting and masking cloud and cloud shadow from satellite remote sensing images is a pervasive problem in the remote sensing community. Accurate and efficient detection of cloud and cloud shadow is an essential step to harness the value of remotely sensed data for almost all downstream analysis. DeepMask, a new algorithm for cloud and cloud shadow detection in optical satellite remote sensing imagery, is proposed in this study. DeepMask utilizes ResNet, a deep convolutional neural network, for pixel-level cloud mask generation. The algorithm is trained and evaluated on the Landsat 8 Cloud Cover Assessment Validation Dataset distributed across 8 different land types. Compared with CFMask, the most widely used cloud detection algorithm, land-type-specific DeepMask models achieve higher accuracy across all land types. The average accuracy is 93.56%, compared with 85.36% from CFMask. DeepMask also achieves 91.02% accuracy on all-land-type dataset. Compared with other CNN-based cloud mask algorithms, DeepMask benefits from the parsimonious architecture and the residual connection of ResNet. It is compatible with input of any size and shape. DeepMask still maintains high performance when using only red, green, blue, and NIR bands, indicating its potential to be applied to other satellite platforms that only have limited optical bands.

==> bios/bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/ke_xu.jpg}}]{Ke Xu} recieved the B.S. degree in Computer Engineering from University of Illinois at Urbana-Champaign, USA, in 2018. He is currently pursuing the M.S. degree in Computer Science at University of Illinois at Urbana-Champaign, USA. His research interests include: computer vision for autonomous driving, vision-aware decision making, human-vehicle interaction, and deep learning for remote sensing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/kaiyu_guan.jpg}}]{Kaiyu Guan} received the B.A. degree in Geography and Geoinformatics from Nanjing University, China, in 2008, and the M.A. and Ph.D. degrees in Water Resources and Environmental Engineering from Princeton University, USA, in 2010 and 2013, respectively. From 2013 to 2015, he was a Postdoctoral Scholar at the Center of the Food Security and the Environment, Stanford University. From 2015 to 2016, he was a Quantitative Scientist with the Climate Corporation. Since 2016, he has been an assistant professor in Ecohydrology and Remote sensing with the Department of Natural Resources and Environmental Sciences, University of Illinois at Urbana-Champaign. He is also a Blue Waters Professor with the National Center for Supercomputing Applications. His research interests include using satellite data, computational models, field work, and machine learning approaches to address how climate and human practices affect crop productivity, water resource availability, and ecosystem functioning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/jian_peng.jpg}}]{Jian Peng} received the B.S. and M.S. degree in Computer Science from Wuhan University, China. He obtained his Ph.D. degree in Computer Science from Toyota Technological Institute at Chicago, USA. He is currently an assistant professor at University of Illinois at Urbana-Champaign, USA. His research interests include: machine Learning, bioinformatics, and machine learning for chemistry.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/yunan_luo.jpg}}]{Yunan Luo} received the B.S. degree from Yao Class at Tsinghua University, China, in 2016. He is currently a Ph.D. student in the Department of Computer Science at University of Illinois at Urbana-Champaign, USA. His research interests include: computational biology and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/sibo_wang.jpg}}]{Sibo Wang} received his B.Sc. degree in Computer Science and Astronomy and his M.S. degree in Environmental Science and Natural Resources, both from University of Illinois at Urbana-Champaign, USA. He currently leads the research activities at Aspiring Universe, a company providing intelligent agriculture solutions. He is interested in applying modern machine learning and high-performance computing methods to precision agriculture and other scientific domains.
\end{IEEEbiography}


% if you will not have a photo at all:
%\begin{IEEEbiographynophoto}{John Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

